A faster FPRAS for #NFA

Given a non-deterministic finite automaton (NFA) A with m states, and a natural number n (presented in unary), the #NFA problem asks to determine the size of the set L(A_n) of words of length n accepted by A. While the corresponding decision problem of checking the emptiness of L(A_n) is solvable in polynomial time, the #NFA problem is known to be #P-hard. Recently, the long-standing open question -- whether there is an FPRAS (fully polynomial time randomized approximation scheme) for #NFA -- was resolved in \cite{ACJR19}. The FPRAS due to \cite{ACJR19} relies on the interreducibility of counting and sampling, and computes, for each pair of state q and natural number i <= n, a set of O(\frac{m^7 n^7}{epsilon^7}) many uniformly chosen samples from the set of words of length i that have a run ending at q (\epsilon is the error tolerance parameter of the FPRAS). This informative measure -- the number of samples maintained per state and length -- also affects the overall time complexity with a quadratic dependence. Given the prohibitively high time complexity, in terms of each of the input parameters, of the FPRAS due to \cite{ACJR19}, and considering the widespread application of approximate counting (and sampling) in various tasks in Computer Science, a natural question arises: Is there a faster FPRAS for #NFA that can pave the way for the practical implementation of approximate #NFA tools? In this work, we demonstrate that significant improvements in time complexity are achievable. Specifically, we have reduced the number of samples required for each state to be independent of m, with significantly less dependence on $n$ and $\epsilon$, maintaining only \widetilde{O}(\frac{n^4}{epsilon^2}) samples per state.

==> applications.tex <==
%!TEX root=./main.tex






\myparagraph{Beyond databases}{
	 \#NFA is a central problem from complexity theoretic perspective. In particular, \#NFA is SpanL-complete and therefore, several problems can be reduced to \#NFA. Therefore, it is no surprise that the \#NFA problem finds applications in a much more wider setting ---
program verification~\cite{SMC2010}, testing of software~\cite{sutton2007fuzzing} 
and distributed systems~\cite{Ozkan2019}, 
probabilistic programming, estimation of information leakage in 
software~\cite{Bang2016,Gao2019,Saha2023},
information extraction~\cite{ACJR21},
automated reasoning using BDDs~\cite{ACJR21},
and even music generation~\cite{Donze2014}.
}


\begin{comment}
\subsection{Applications of Automata Counting}
\seclabel{applications}

\myparagraph{Regular Path Queries in Graph Databases}{
Regular path queries (or \emph{property paths}) form a rich fragment of graph query languages used in graph database systems.
Here, one abstracts information on edges in the graph database using an alphabet $\alphabet$
and asks a variety of questions about the set of paths that start from a given source node $u$,
end at a target node $v$.
In particular, a regular path query $(u R v)$ asks to 
enumerate, count or uniformly sample the set of paths (bounded in length
by some fixed number $n$) from $u$ to $v$
whose labels match the regular expression $R$.
Often, $R$ is a generic regular expression and cannot be compiled to a polynomially longer DFA.
Likewise, in absence of any domain-specific restrictions, the database in question allows for non-determinism (i.e., a node maybe adjacent to multiple nodes through the same label $\sigma \in \alphabet$).
In these settings, one can naturally the counting/sampling problems of the above kind to the \#NFA
problem, for the NFA obtained by the cross product of NFA represented by the database (with $u$ as the intial state and $v$ as the final state) and the NFA that $R$ gets compiled down to.
This reduction is \ucomment{linear} in the size of the database as well as the query and thus an efficient approximation scheme for \#NFA can also be used to answer counting and sampling questions for regular path queries. \ucomment{citations}
}

\myparagraph{Conjunctive Queries and Probabilistic databases}{
An efficient solution for approximating \#NFA 
can also be used to answer the probabilistic query evaluation 
problem (alternatively, computing the uniform reliability measure) 
for probabilistic graph databases.
This is specifically true for the simple case of a conjunctive path queries of the form
$\varphi = R_1(x_1, x_2), R_2(x_2, x_3) \ldots, R_n(x_n, x_{n+1})$,
where $R_i$s are binary relations in the underlying relational schemum.
The measure of the query $\varphi$ against a probabilistic database $D$
is the total measure of each sub-database $D' \subseteq D$ for which $\varphi \models D'$;
here the measure of $D'$ is simply the product of the probabilities
$p_f$ (resp. $1-p_f$) associated with each record $f$ that occurs in $D'$ 
(resp. does not occur in $D'$).
While exact computation of the uniform reliability measure of a probabilistic database is a \#P-hard problem, recent results obtain a FPRAS for it by reducing it into an instance of \#NFA
whose size is \ucomment{linear} in the size of the query $\varphi$
and \ucomment{linear} in the size of the database $D$.
Clearly, a faster FPRAS for \#NFA can be used to speed up the task of approximating the uniform reliability measure.
\ucomment{citations.}
}

\myparagraph{Beyond databases}{
The \#NFA problem finds applications 
in program verification~\cite{SMC2010}, testing of software~\cite{sutton2007fuzzing} 
and distributed systems~\cite{Ozkan2019}, 
probabilistic programming, estimation of information leakage in 
software~\cite{Bang2016,Gao2019,Saha2023},
information extraction~\cite{ACJR21},
automated reasoning using BDDs~\cite{ACJR21},
and even music generation~\cite{Donze2014}.
}
\end{comment}

==> motivating.tex <==
%!TEX root=./main.tex

\section{Applications of Automata Counting and Sampling}
\seclabel{motivation}

In this section, we illustrate the applications of 
counting and sampling in various domains in Computer Science,
including testing and verification, for readers
that may otherwise be less familiar.

\subsection{Randomized Testing With Probabilistic Guarantees}

While full-fledged formal verification
of large scale software often involves several person-years of effort
by dedicated experts~\cite{hawblitzel2015ironfleet},
randomized testing techniques such as fuzz testing~\cite{sutton2007fuzzing}, 
controlled concurrency testing~\cite{CCT2016,Coyote2023,PCT2010}
and constrained random simulation-based functional 
verification~\cite{CRV2007} have emerged as powerful 
means to ensure reliability of such systems. 
Randmized techniques have successfully been applied
to testing of distributed key-value stores~\cite{Ozkan2019}, 
pre-Silicon processor designs~\cite{Chakraborty2020} and have also 
uncovered security vulnerabilities in the Linux kernel~\cite{xu2020krace,Razzer2019}.
While such randomized techniques are largely heuristic driven,
those backed with systematic sampling techniques often shine,
both in terms of their formal coverage guarantees as well as their
empirical coverage~\cite{Ozkan2019,PCT2010,WMMPCT2023}.
A crucial component in the latter algorithms is the capability
to sample executions from a given set (typically all paths of a program)
\emph{uniformly} at random.
The rationale behind the choice of uniformity in the sampling procedure 
is simple --- bugs hide in unknown places
and a strategy that explores a diverse set of behaviors is likely
to find deep bugs than a biased directed search.

\input{figures/cfg}

In the setting of randomized testing, the system under test is modeled using a finite state
transition system, also known as the \emph{control flow automaton} of the system,
and looks similar in shape to the \emph{control flow graph} of the program.
The control flow automaton is a syntactic abstraction of the program;
we illustrate this using an example in~\figref{prog-cfg}.
The states of the automaton (see for example $\ell_\texttt{1}, \ell_\texttt{7}, \ell_\texttt{exit}$ in~\figref{cfg}) correspond to the 
program locations of the program being modeled (see for example \figref{prog}).
The transitions are labeled with program statements (assignments or conditions)
and are typically treated as syntactic labels alone.
The alphabet can be chosen to be the set of labels on states, 
labels on transitions or both.
Each (labeled) path in the automaton corresponds to a word,
and further multiple paths may correspond to the same word
i.e., the control flow automaton may, in general, be non-deterministic,
especially when constructs like external library calls or complex expressions
are not modeled explicitly.
All or some states may be marked accepting.
The uniform sampling question then asks to generate all labeled paths in the control flow
automaton whose length is some fixed number $n$.



\subsection{Quantitative Information Flow}

Security-critical components (such as password checkers) 
in most user-facing software applications are often the Achilles' heel,
from the perspective of security vulnerabilities.
Software developers 
\input{figures/qif}  
\noindent therefore often need to make careful
design and implementation decisions to ensure that the amount
 of
information leakage based on side-channels such as timing and energy characteristics
are minimized.
Quantification of the information leakage in software can often prove to be
an important tool at the disposal of security-conscious developers
who compare different functionally-equivalent implementations that differ in the amount of information they leak.
Shannon entropy~\cite{Millen1987} and min-entropy~\cite{Smith2009} have
emerged as popular metrics for measuring information leakage.
While both metrics have subtle differences, they share a common computational aspect --- counting.
We focus on Shannon entropy for the sake of illustration.
Consider the Python program in \figref{qif} that validates a candidate password.
Assuming the input password is secret information,
measuring the Shannon entropy of this program boils down to measuring,
for each output $o$, the number of inputs that correspond to the output $o$.
Here for example, this amounts to counting, for each return code amongst
$r \in \set{\texttt{ERR\_URL}, \texttt{ERR\_ALPHANUM}, \texttt{ERR\_PII}, \texttt{ERR\_LEN}, \texttt{PASS}}$,
the number of input strings that map to $r$.
For the return code $r = \texttt{PASS}$,
observe that the set of strings that map to $r$ are precisely those strings
that belong to the regular language $L_{\texttt{PASS}} = \setpred{w \in \Sigma^*}{8 \leq |w| \leq 20, w \neq \texttt{phone}, w \not\in L_\texttt{URL}, w \in L_\texttt{ALPHANUM}}$.
In fact, all the return codes correspond to regular languages,
and the task of estimating Shannon entropy essentially boils down to counting
the number of strings (of lengths bounded by, say some maximum length $M$) in each of these regular languages.
Prior works~\cite{Bang2016,Gao2019,Saha2023} often generate string constraints
using symbolic execution and rely on automata counting techniques~\cite{Aydin2015,Trinh2017} for
estimating information leakage.


% \subsection{Probabilistic Symbolic Execution}

% \subsection{Statistical Model Checking}

\subsection{Machine Improvisation of Music}


An interesting application for sampling from regular languages is
in the field of machine 
\input{figures/music}
\noindent
improvisation~\cite{rowe2004machine},
which studies the use of data-driven and rule-based methods for automated
 generation of melodies.
A classic approach here is to generate variants
obtained by extracting patterns from a reference melody,
which can then be combined repeatedly.
In recent efforts to give a formal treatment to the problem of
music improvisation, the use of formal languages have been proposed~\cite{Donze2014,Valle2016}.
In this setting, melodies are treated symbolically and modeled
as words over a fixed alphabet $\Sigma$, 
often described as a cartesian product of several alphabets (`pitches', `durations', `chords', `beats'~\cite{Donze2014}).
The space of melodies is often derived from a reference melody $w_\textsf{ref} \in \Sigma^*$,
by constructing what is called as the `Factor Oracle' $\mathcal{O}$
improviser obtained from $w_\textsf{ref}$. 
Often $\mathcal{O}$ is an NFA, whose size grows
with the size of the reference melody $w_\textsf{ref}$.
Additionally, a space of safe specifications, also represented using a formal language
such as a regular language encoded using an automaton $\aut_\textsf{safe}$,
is provided.
Regular safety specifications can encode requirements such as `note $a$ is always followed by $3$ occurences of note $b$'
or `chords $C$ and $A$ alternate'.
Finally, the task of music generation asks to generate melodies close to the reference melody
subject to the constraints of safety, while ensuring variety
in the generative process.
This can formally be modeled as
the task of uniformly (or approximately-uniformly) 
sampling from the language $\lang{\mathcal{O}} \cap \lang{\aut_\textsf{safe}}$.



==> overview.tex <==
%!TEX root=./main.tex

\section{Overview of the FPRAS algorithm}

On a high-level, our approach follows a template similar to that of Arenas et al.~\shortcite{ACJR21}: we rely on the self-redubility of NFA and inter-reducibility of approximate counting and uniform sampling. 
Consequently, our algorithm fits the template algorithm outlined in~\cite{ACJR21}: for each state $q$ and path length $\ell \leq n$, we incrementally maintain an estimate, $N(q^{\ell})$, of $|\lang{q^{\ell}}|$. 
To estimate $N(q^{\ell})$, we rely on the estimates of  $\lang{p^{\ell}}$ for all $q$ for which is transition $(p,\bb,q) \in \aut$, where $\bb \in \{0,1\}$. Observe that 
\begin{align*}
 \lang(q^{\ell}) = 0\cdot\cup_{(p,0,q)\in \trans} \mathcal{L}(p^{\ell-1}) \bigcup 1\cdot\cup_{(p,1,q)\in \trans } \mathcal{L}(p^{\ell-1}).   
\end{align*}

It is worth remarking that  $\mathcal{L}(p^{\ell-1})$ may not be disjoint for different $p$. To this end, we rely on maintaining a set, $S(p^{\ell-1})$ for each $p$, of samples of strings belonging to $\lang{p^{\ell-1}}$. Ideally, one would like the set $S(p^{\ell-1}$ to be composed of strings $w$ sampled uniformly at random. To this end, we can rely on the self-reducibility property, i.e., we can first partition $\lang{p^{\ell-1}}$ into the set of strings with the last character being $0$ or $1$, and accordingly sample the last character, and then recursively sample the bits one by one, i.e., we can sample by growing suffix of $w$. Finally, we need to account for the  errors that propagate in the estimates of $N(q^{\ell})$. 

While on a high level, our approach is similar to that of~\cite{ACJR21}, there are crucial technical details that allow us to obtain FPRAS with significantly lower time complexity. To this end, the crucial underlying invariant in ~\cite{ACJR21} is to ensure that the following condition holds at every level $\ell$, for $\kappa = \frac{nm}{\varepsilon}$: 

\begin{align}\label{eq:acjrcond}
   \xi(\ell) := \forall q \in Q \; \forall P \subseteq Q \; \big\vert 
   \frac{|S(q^{\ell}\setminus \cup_{p \in P} \lang{p^{\ell}}|}{|S(q^{\ell})|}
   -
   \frac{|\lang{q^{\ell}}\setminus \cup_{p \in P} \lang{p^{\ell}}|}{|\lang{q^{\ell}}|} \big\vert \leq \frac{1}{\kappa^3} 
\end{align}

In other words,  ~\cite{ACJR21} would like to have an $\frac{1}{\kappa^3}$-additive approximation for  $\frac{|\lang{q^{\ell}}\setminus \cup_{p \in P} \lang{p^{\ell}}|}{|\lang{q^{\ell}}|}$ for every $q \in Q$ and $P \subseteq Q$.  From standard concentration bounds, we know that such an additive approximation (with probability $\eta$)  for a given $q$ and  $P$ would be possible if the size of $|S(q^{\ell})|$ is  $O(\frac{k^6}\log \eta^{-1})$ . Since we would like to ensure that we have an additive approximation for all $q$ and $P$, we would be dealing with union bounds over exponentially many events, and accordingly it is advisable to have $\delta^{-1} = O(2^{mn})$, and consequently, ~\cite{ACJR21} maintain $O(k^7)$ samples for each state $q$.  Ensuring  $\xi(\ell)$ to hold at every level, allows ~\cite{ACJR21} to show that, conditioned $\xi{i}$ for all $i \leq \ell$, it is possible to sample every element  of $\lang{q^{\ell}}$ uniformly at random.

This raises the question: what should one do to lower the requirement on the size of $S(q^{\ell})$? Our approach is to identify a significantly weaker condition, called $\accurateEstevent_{q, \ell}$, to hold true instead of $\xi(\ell)$. In particular, $\accurateEstevent_{q, \ell}$ refers to ensuring  that for every state $q$ and level $\ell$, we can obtain an estimate  $N(q^{\ell})$ that is a $(1+\frac{\varepsilon}{2n^2})$-approximation of $|\lang{q^{\ell}}|$. 
It is worth remarking that analysis of ~\cite{ACJR21} shows that  $\xi(\ell)$ implies $\accurateEstevent_{q, \ell}$. Observe that for $\accurateEstevent_{q, \ell}$ to hold with  probability $\eta$, $O(\frac{n^4}{\varepsilon^2})\log \eta^{-1}$ samples suffice. Furthermore, we have to now perform a union bound only over $O(mn)$ many events, and therefore, $\eta^{-1} = O(mn)$ suffices. There is, of course, no free lunch: it is no longer the case that  conditioned on $\accurateEstevent_{q, \ell}$, we can ensure every element  of $\lang{q^{\ell}}$i is sampled uniformly at random. Fortunately, we do not need such a strong condition, it suffices to have the distribution of $S(q^{\ell})$ be close to the set of uniformly chosen samples in statistical distance.  Fortunately, we can still rely on self-reducibility to construct $S(q^{\ell})$. It is worth remarking that given our reliance on weaker condition, our procedure to estimate $N(q^{\ell})$ also differs from that of ~\cite{ACJR21}, and to this end, we rely on adaptation of a recent result of Meel\textcircled{r}Vinodchandran\textcircled{r}Chakraborty for computation of union of sets. 


Given the high-level similarity of the two approaches, the time complexity of the approaches can be presented as $O(n \cdot (m\cdot n) \cdot (m+n) \cdot \cdot |S(q^{\ell})|^2)$ where the first $n$ from the length of every string,  the factor $(m \cdot n)$ corresponds to the upper bound on the number of states in the unrolled automaton, and the factor $(m+n)$ corresponds to the time taken for membership check. Accordingly, it is instructive to compare the bound of $O(\frac{m^7 n^7}{\varepsilon^7})$ for  $|S(q^{\ell})|$ in ~\cite{ACJR21} to  $O(\frac{n^2}{\varepsilon})$ in our approach. In particular, the number of samples for every state in our approach is independent of $m$. 


==> related.tex <==
%!TEX root=./main.tex

\section{Related Work}
\seclabel{related}
The problem of enumerating strings of length $ n $ (expressed in unary) that are accepted by a non-deterministic finite automaton (NFA) is fundamental in various disciplines. Developing efficient Fully Polynomial Randomized Approximation Scheme (FPRAS) algorithms for this task has long been challenging. This problem is established as \#P-complete \cite{ALVAREZ19933}, and until recently, the predominant algorithm could only offer quasi-polynomial time randomized approximation schemes (QPRAS) \cite{GoreJKSM97, KannanSM95}. A significant breakthrough, however, was achieved by Arenas, Croquevielle, Jayaram, and Riveros \cite{ACJR21}. Their proposed stores for each state $ p$ in the NFA and for each string length $\ell$ (ranging from 0 to $ n $), a sample of strings from $\mathcal{L}(p^{\ell}$. This method maintains a sample size of $ O(\kappa^7) $, where $ \kappa = O(nm/\epsilon) $ and $ m $ is the number of states in the NFA.

The algorithm advances by calculating the sample set for a given $ p $ and $ \ell $ using previously computed sample sets. For each sample, it is necessary to compute the union of sampled sets for a subset of states, leading to a total generation cost for a single sample set of $ O(m \cdot s^2) $, with $ s $ being the sample set size, which is $ O(\kappa^7) $. Collectively, their proposed FPRAS scheme exhibits a time complexity of $ O\left(\frac{m^{16} \cdot n^{17}}{\varepsilon^{14}}\log (1/\delta)\right) $.




